I Always Feel Like Somebody's Sensing Me! A Framework to Detect, Identify, and Localize Clandestine Wireless Sensors

The increasing ubiquity of low-cost wireless sensors has enabled users to easily deploy systems to remotely monitor and control their environments. However, this raises privacy concerns for third-party occupants, such as a hotel room guest who may be unaware of deployed clandestine sensors. Previous methods focused on specific modalities such as detecting cameras but do not provide a generalized and comprehensive method to capture arbitrary sensors which may be "spying" on a user. In this work, we propose SnoopDog, a framework to not only detect common Wi-Fi-based wireless sensors that are actively monitoring a user, but also classify and localize each device. SnoopDog works by establishing causality between patterns in observable wireless traffic and a trusted sensor in the same space, e.g., an inertial measurement unit (IMU) that captures a user's movement. Once causality is established, SnoopDog performs packet inspection to inform the user about the monitoring device. Finally, SnoopDog localizes the clandestine device in a 2D plane using a novel trial-based localization technique. We evaluated SnoopDog across several devices and various modalities and were able to detect causality for snooping devices 95.2% of the time and localize devices to a sufficiently reduced sub-space.

==> Sources/rebuttal.tex <==
\section{Author Response (List of Changes)}\label{sec:rebuttal}

We thank the reviewers for their insightful comments and valuable suggestions. As soon as our lab re-opened under COVID-19 restrictions, we purchased additional hardware to expand upon our experiments and evaluation as suggested by the reviewers. In addition, we re-wrote the paper to clarify and elaborate on the topics introduced by the reviewers.

\subsection{Writing}
\noindent\textbf{\textit{1. Addressing novelty} (Reviewer \#221A)}. 
\begin{itemize}
    \item \namenospace, to the best of our knowledge, is the first generalized framework to detect hidden clandestine sensors, including video, audio, motion, and RF. \name leverages the cause-effect relationship between a trusted set of sensor values and \wifi traffic patterns when observing a multi-modal injected event.
    \item We present a novel technique that leverages the notion of directional sensor coverage to provide state-of-the-art localization for clandestine devices.
\end{itemize}

\noindent\textbf{\textit{2. Addressing assumptions in the adversarial model} (Reviewer \#221A)}. 

We focus on adversaries whose goal is to remotely spy on a third-party occupant of a private space in real-time. This model is consistent with other state-of-the-art methods for detecting hidden cameras~\cite{cheng2018dewicam,wampler2015information,nassi2019drones,liu2018detecting}, and is supported anecdotally by several cases where owners were live-streaming guests in private spaces, e.g., \cite{airbnb-news, jeong_griffiths_2019}. Further, many commercially available devices do not offer a local storage option for reasons of size, weight, power, and cost -- such is the case with six out of the popular twelve devices we examined. Moreover, live-streaming offers a more practical and scalable solution from a management perspective. Thus, we assume the adversary uses an arbitrary set of wireless, commercial-off-the-shelf (COTS) sensors that are tailored for clandestine placement. An adversary may use one of the several techniques mentioned in Appendix \ref{sec:appendix-fool} to fool \namenospace, for example with cover traffic or local storage. Implementing these techniques can require modifying the device firmware or physically interfacing with a proxy device (e.g., RPi), thereby increasing the barrier-to-entry for potential attackers. Moreover, techniques such as cover traffic can add significant and undesirable network overhead, particularly for a large number of sensors.

\noindent\textbf{\textit{3. ``Pack the first 4 pages more tightly”} (Reviewer \#221A)}. 

We have re-written the introduction, background, and system overview to eliminate redundancy and concisely highlight the research contributions. We have also restructured the background section to elucidate the notions of causality that were previously introduced in the design section. The notion of causality provides a foundation for understanding the system and adversary models and provides preliminary insight as to how we can establish causality between trusted sensor values and WiFi traffic patterns.

\noindent\textbf{\textit{4. Justification for sensors used} (Reviewer \#221B)}.
\begin{itemize}
    \item We have tested our framework on some of the most commonly used sensors in smart home settings~\cite{amazoncameras, amazonhomeautomation}. These sensors include cameras, smart home assistants, motion sensors, and RF sensors.
    \item The specific devices and sensors we have used are some of the best-sellers and most popular ones in their category. We demonstrated our framework on some of the most well-known brands including Amazon (Ring), Samsung, Google, Arlo (Netgear), and Panasonic.
\end{itemize}

\noindent\textbf{\textit{5. Tone down the contributions and be forthcoming with the limitations.} (Reviewer \#221D)}

We have re-written major parts of the paper and have added more evaluation to bring out the limitations of our work. We have also added a discussion of all the limitations and trade-offs of our work. The sections include: Abstract, Introduction, Overview, Discussion, and Evaluation.

\noindent\textbf{\textit{6. Demonstrate SnoopDog’s ability to work on other IoT protocols such as ZigBee and RF. Here, please justify how to get readily available monitoring equipment to cover the wireless domain.} (Reviewer \#221E)}
\begin{itemize}
    \item We have reduced the scope and contribution of SnoopDog to WiFi-based sensors only.
    \item In certain cases, sensors that use Zigbee and ZWave in smart home settings interface with the cloud using a WiFi hub. We can sniff the traffic of this WiFi hub to determine if sensors are monitoring the user. To show this, in our expanded evaluation we purchased a Samsung Smart Home motion sensor that uses ZWave through a WiFi hub and determined that our approach can work for such sensors.
    \item Additionally, we have added a new section in the discussion section on recent works that capture Zigbee and ZWave traffic through WiFi cards using cross-technology communication. As these techniques become more mature, we hope to expand the scope of our work.
\end{itemize}

\noindent\textbf{\textit{7. How to deal with MAC randomization?} (Reviewer \#221B)}

In order to deal with techniques such as MAC randomization, we can use techniques such as the ones described here~\cite{vanhoef2016mac}. We can first de-randomize traffic for each individual device and then run our analysis on it.  We have added this to our paper as well.

\subsection{Evaluation}
\noindent\textbf{\textit{8. Add evaluation of multiple popular brands of additional sensors and IoT systems. Please also evaluate popular brands of cameras.} (Reviewer \#221E)}
\begin{itemize}
    \item We bought cameras from well-known brands such as Panasonic, Netgear (Arlo), and Ring (Amazon). We also bought a Google Home Mini and a Samsung Smart Things motion sensor. We ran our trials for these cameras and empirically demonstrated that SnoopDog can work well on them.
    \item The reviewers had asked us to test our framework on a Sony camera. We tried to purchase a wireless IP camera from Sony. Unfortunately, as of 31st August 2020, Sony does not list a wireless IP camera on its website \href{https://pro.sony/ue_US/products/ip-cameras}{(Click Here)}. It had produced one wireless IP camera in past \href{https://pro.sony/ue_US/products/ip-cameras/video-security-wifi-networking-snccx600w-security-camera}{(Click Here)} but it has since been discontinued. We procured a camera from another aftermarket website. Unfortunately, even after our best efforts, we could not make the camera work properly. The video was very choppy which could be due to the drivers not being updated. Hence, we have not shown our results on this camera.
\end{itemize}

\noindent\textbf{\textit{9. For Alexa drop-in features, please show the evaluation of home traffic changes as a function of user speech vs. quiet room (as opposed to accidentally stumbling on the wake word). Showing that this works on other assistants such as Google’s and Apple’s will further add strength to the paper’s results.} (Reviewer \#221E)}
\begin{itemize}
    \item We procured a Google Home Mini and demonstrated that our framework works for it as well.  These results are included in our expanded evaluation.
    \item We performed additional experiments to show traffic changes as a function of human speech for Alexa Drop-In. This is available in Appendix~\ref{sec:drop_in}.
\end{itemize}

\noindent\textbf{\textit{10. Empirically demonstrate SnoopDog on H.264/MPEG-4 codecs} (Reviewer \#221E)}

All the cameras we have experimented on use H.264/MPEG-4 codecs, therefore showing that our approach works on codecs of this family. This has been made clear in the evaluation.


\noindent\textbf{\textit{11. Empirically demonstrate the need for an additional sensor triggered by the user, as opposed to passively analyzing network traffic.} (Reviewer \#221E)}

We have added a new evaluation+discussion section (Section~\ref{sec:discussion}-Q9): The Impact of a Ground Truth Sensor) where we empirically demonstrate that a ground truth sensor can significantly reduce the rate of false positives. We have also added an example figure demonstrating the same. The addition of a ground truth sensor reduces the likelihood of classifying innocuous sensors as spying on the user. 

\noindent\textbf{\textit{12. Expand your experiments to understand the trade-offs of the system.} (Reviewer \#221D)}
\begin{itemize}
    \item In section~\ref{sec:false-positive}, we added an evaluation of the false-positives of the background phase, which requires minimal user overhead, with the active phase.
    \item We also added a discussion detailing the impact of several simultaneous clandestine sensors and the addition of multiple radios to improve the overall system performance.
\end{itemize}
